Working hard to know your neighbor's margins: Local descriptor learning loss

We introduce a novel loss for learning local feature descriptors which is inspired by the Lowe's matching criterion for SIFT. We show that the proposed loss that maximizes the distance between the closest positive and closest negative patch in the batch is better than complex regularization methods; it works well for both shallow and deep convolution network architectures. Applying the novel loss to the L2Net CNN architecture results in a compact descriptor -- it has the same dimensionality as SIFT (128) that shows state-of-art performance in wide baseline stereo, patch verification and instance retrieval benchmarks. It is fast, computing a descriptor takes about 1 millisecond on a low-end GPU.

==> commented_out.tex <==

%\subsection{Quadruplet loss}
%\begin{enumerate}
%\item 
%\end{enumerate}
%\label{main:quadruplets}
%Our core idea is to combine strength of both approaches to create state-of-the-art solution for matching problem. This approach consists of two parts: adding SIFT descriptor to the network output in residual style and learn ranking - distance in-between "easy" and "hard" patches as a part of network by adding restrictions not only for positive-negative images, but for distance from 'easy' positive image (any positive image of the viewpoint) to "hard" positive images. 
"Hard" images were received by adding geometrical and illumination augmentation to the positive images.

The most of learned CNN-based local descriptors rely on siamese architecture with contrastive or triplet margin loss. In case of contrastive loss networks sees two patches and Eucledian distance between should satisfy condition 1:

d(q,same) <= margin
d(q, neg) > margin

For triplet margin loss condition is like this:

d(q,n) - d(q,s) > margin. 


And the common evaluation is false positive rate(FPR) at point of 0.95 true positive recall. The state of art is 4\% for . Recently ~\cite{TFeat2016} have been experimentally shown that good performance on patch verification task does not always imply good performance in nearest neighbors setup, which is used for image matching. 
Local features are detected by detector like DoG, MSER of Hessian-Affine, 500..5000 features per image and descripted by descriptor. Then for each feature F1 in image 1 nearest neighbor in image F2 is found. 
The probability that at least one false postitive (feature with distance less than threshold is ), if the FPR is 4\%.  

With FPR = 4\% and average number of features per image ~4000, the expectation of false positives is ~4.smth features. Althought, it is not yet failure, if distance to the correct neighbor is smaller than to the false positives. But the task of sorting patches by similarity inside of threshold radius is not used during learning and outcome is, in fact, random. 

Therefore we propose to fix this problem by introducing additional auxiliary loss.












All patches are normalized by substracting mean and standard deviation computed from the training set. 

As a baseline we've taken siamese triplets network architecture described in \cite{tfeat}, which was known to provide better results that it's previous antecedents.
Our best performance was achieved on siamese quadruplets architure, that is shown at Fig. 1.

First thing to mention is the generation of "hard" positive images: we take anchor, find any positive patch of the same keypoint and generate "hard" positive image using augmentation procedure. Augmentation procedure helps us to take control on "hard" images generation and works as follows: random crops (params are here), random gaussian blur (params are here), random (params are here).  

Also, we propose to add "hard-positive" margin loss to teach network ranking not only within positive-negative pairs as descibed in \cite{tfeat}, but also in-between positive pairs, which is similar to matching task. "Hard-positive" margin was chosen as 0.25 as it showed good results even without further optimization. 

Our model was trained with procedure in \cite{tfeat} on 5M quadruplets pre-generated from \cite{PhotoTourism} dataset. For each anchor patch random patch from the same physical point was extracted and random patch from and negative point within dataset from one location. Training is done with batch size 128. Stochastic Gradient Descend was used for optimization with initiali learning rate of 0.1 that was reduced every epoch on 0.05.




Convolutional neural network architecture is show at Fig.1. SIFT is used as a part of network. \cite{keras_sift} In comparison with \cite{tfeat} one more convolutional and pooling layers were added to the network. Also, output of the last convolutional layer was normalized with l2 layer. 
SIFT is added to the network as a addition to the convolutional output, which allows us to say that we train network in residual style. 
Several different architectures were tried among which this one shown itself as the best.

Classification: ROC AUC, PR AUC

Matching: Algorithm, described in \cite{WxBS_dataset}



\begin{figure}[htbp]
\includegraphics[width=0.35\textwidth]{images/network_architecture1_1.png}
\includegraphics[width=0.55\textwidth]{images/network_architecture1_2.png}

\caption{Siamese quadruplets network architecture}
\label{fig:siamese_quadruplets_topology}
\end{figure}




==> hpatches_table.tex <==

\begin{table}[htb]
\centering
\caption{Performance on HPatches dataset with PCA-whitened descriptors. All learned descriptors were trained on \textit{Liberty} sequence~\cite{Brown2007}. + stands for augmentation: random rotation on 90 degrees and flip.}
\label{matching3}
\begin{tabular}{lllll}
 \hline
Descriptor        & Easy   & Hard   & Tough  & Mean   \\
\hline
MinDistNet+        & 0.6717 & 0.4948 & 0.3153 & 0.4939 \\
MinDistNet      &  0.6372&	0.4545&	0.2843&	0.4587 \\
L2Net+     & 0.6168 & 0.4269 & 0.2585 & 0.4341 \\
L2Net          & 0.5777 & 0.3698 & 0.2100 & 0.3858 \\
TFeat             & 0.5969 & 0.3079 & 0.1557 & 0.3535 \\
RootSIFT          & 0.5540 & 0.2701 & 0.1306 & 0.3182 \\
%SIFT              & 0.5398 & 0.2748 & 0.1390 & 0.3179
\end{tabular}
\end{table}




\begin{table}[htb]
\centering
\caption{Performance on HPatches dataset. All learned descriptors were trained on \textit{Liberty} sequence~\cite{Brown2007}. + stands for augmentation: random rotation on 90 degrees and flip. }
\label{tab:matching2}
\begin{tabular}{@{}ccccc@{}}
\toprule
Descriptor        & Easy   & Hard   & Tough  & Mean   \\
\hline
MinDistNet+    & 0.6629&	0.4824&	0.3066	&0.4840\\
MinDistNet    &  0.6212&	0.4399	&0.2727&	0.4446 \\
L2Net+     & 0.6142 & 0.4286 & 0.2606 & 0.4345 \\
L2Net         & 0.5831 & 0.3782 & 0.2180 & 0.3931 \\
TFeat             & 0.4999 & 0.2748 & 0.1390 & 0.3046 \\
RootSIFT          & 0.4815 & 0.2087 & 0.0935 & 0.2613 \\
%SIFT              & 0.4532 & 0.1930 & 0.0863 & 0.2442
\end{tabular}
\end{table}




\begin{table}[htb]
\centering
\caption{Verification performance on HPatches dataset. Inter - contains negative pairs sampled from between sequences.}
\label{tab:hbench_verification1}
\begin{tabular}{lllllll}
\hline
Metric            & \multicolumn{3}{c}{AUC}        & \multicolumn{3}{c}{AP}         \\
Descriptors       & Easy     & Hard     & Tough    & Easy     & Hard     & Tough    \\
\hline
SIFT              & 0.93 & 0.82 & 0.73 & 0.85 & 0.66 & 0.51 \\
RootSIFT          & 0.90 & 0.80 & 0.72 & 0.78 & 0.58 & 0.37 \\
TFeat-margin      & 0.96 & 0.94 & 0.90 & 0.92 & 0.85 & 0.75 \\
L2Net             & 0.97 & 0.93 & 0.87 & 0.93 & 0.85 & 0.74 \\
L2Net+      & 0.97 & 0.94 & 0.89 & 0.94 & 0.88 & 0.78 \\
MinDistNet        & 0.97 & 0.94 & 0.89 & 0.94 & 0.88 & 0.77  \\
MinDistNet+ & 0.98 & 0.95 & 0.90 & 0.95 & 0.89 & 0.80 \\  
\end{tabular}
\end{table}

\begin{table}[htb]
\centering
\caption{Verification performance on HPatches dataset. Intra - contains negative pairs sampled from withing sequences.}
\label{tab:hbench_verification1}
\begin{tabular}{lllllll}
\hline
Metric            & \multicolumn{3}{c}{AUC}        & \multicolumn{3}{c}{AP}         \\
Descriptors       & Easy     & Hard     & Tough    & Easy     & Hard     & Tough    \\
\hline
SIFT              & 0.91 & 0.80 & 0.71 & 0.78 & 0.57 & 0.43  \\
RootSIFT          & 0.88 & 0.76 & 0.68 & 0.69 & 0.48 & 0.37 \\
TFeat-margin      & 0.95 & 0.91 & 0.86 & 0.87 & 0.78 & 0.67 \\
L2Net             & 0.96 & 0.93 & 0.87  & 0.92 & 0.83 & 0.72 \\
L2Net+            & 0.97 & 0.94 & 0.88 & 0.93 & 0.86 & 0.75 \\
MinDistNet        & 0.96 & 0.93 & 0.87  & 0.92 & 0.84 &  0.72 \\
MinDistNet+ 	  & 0.97 & 0.94 & 0.88 & 0.92 & 0.86 & 0.75
\end{tabular}
\end{table}
